Traversable Wormholes, Regular Black Holes, and Black-Bounces

Various spacetime candidates for traversable wormholes, regular black holes, and `black-bounces' are presented and thoroughly explored in the context of the gravitational theory of general relativity. All candidate spacetimes belong to the mathematically simple class of spherically symmetric geometries; the majority are static, with a single dynamical (time-dependent) geometry explored. To the extent possible, the candidates are presented through the use of a global coordinate patch -- some of the prior literature (especially concerning traversable wormholes) has often proposed coordinate systems for desirable solutions to the Einstein equations requiring a multi-patch atlas. The most interesting cases include the so-called `exponential metric' -- well-favoured by proponents of alternative theories of gravity but which actually has a standard classical interpretation, and the `black-bounce' to traversable wormhole case -- where a metric is explored which represents either a traversable wormhole or a regular black hole, depending on the value of the newly introduced scalar parameter $a$. This notion of `black-bounce' is defined as the case where the spherical boundary of a regular black hole forces one to travel towards a one-way traversable `bounce' into a future reincarnation of our own universe. The metric of interest is then explored further in the context of a time-dependent spacetime, where the line element is rephrased with a Vaidya-like time-dependence imposed on the mass of the object, and in terms of outgoing\-/ingoing Eddington-Finkelstein coordinates. Analysing these candidate spacetimes extends the pre-existing discussion concerning the viability of non-singular black hole solutions in the context of general relativity, as well as contributing to the dialogue on whether an arbitrarily advanced civilization would be able to construct a traversable wormhole.

==> 05-Generalised-TW.tex <==
\chapter{The generalised traversable wormhole}\label{C:GeneralisedTW}

%%%%%%

\section{The generalised static and spherically symmetric traversable wormhole} \label{generalextension}

\blue {(taken from morris-thorne section - adapt appropriately...)} This metric corresponds to a one-chart atlas, \emph{i.e.} a global coordinate patch covering both universes (it is easily seen that the metric is anlaytic for all $r\in(-\infty, +\infty)$). In Lorentzian Wormholes \cite{LorentzianWormholes}, it is detailed how one can exte nd this simple construction to a more general case for an arbitrary static, spherically symmetric traversable wormhole geometry using \textbf{two} coordinate patches (essentially one for each universe). This approach has sometimes been considered amongst some researchers as implying that in order to conduct useful, tractable analysis on a traversable wormhole geometry, one must have an atlas with multiple charts \footnote{Names suppressed to protect the guilty}. It is therefore of interest to analyse a generalised metric for the static, spherically symmetric case which is covered by a global coordinate patch, and observe the results.

The metric can, w.l.o.g, be defined as follows:

\begin{equation}
    ds^2 = -F(r)dt^2+G(r)dr^2+\left(r^2+a^2\right)\left(d\theta^2+\sin^2\theta d\phi^2\right) \ .
\end{equation}

Note that $\xi=\lbrace\partial_{t}, \partial_{\phi}\rbrace$ is a hypersurface orthogonal timelike Killing vector field, hence the metric is static, and in view of the diagonal metric environment it is also clearly spherically symmetric as supposed.

\noindent We may immediately introduce some conditions on the coefficient functions $F(r)$ and $G(r)$. In order for this to correspond to a traversable wormhole geometry, by definition we must have no event horizons present and so $F(r)$ must be everyhwere non-zero. A traversable wormhole geometry also has the property that in each universe on either side of the wormhole throat, the geometry must possess an asymptotically flat region. It follows naturally that these regions will be at coordinate locations $r=\pm\infty$ respectively. \red {(keep listing the natural properties required for trav. wormhole geometry (see pgs 101-102 L.W. for details).... probably an itemise here is best, and potentially an introductory paragraph earlier prior to introducing any metrics detailing exactly what a trav. wormhole geometry requires)}

\red {(Include refractive index, coordinate speed of light here)}

%

\subsection {Curvature tensors and curvature invariants analysis:}

\red{to be completed... working on while away}
%

\subsection {ISCO and photon sphere analysis:}

Of immediate interest when analysing our generalised traversable wormhole geometry are the necessary and sufficient conditions for the existence of an ISCO or photon sphere location within our own universe. Physically, we would like a sensible coordinate location for both of these things so that astronomers may better know where to search for accretion disks for various black hole candidates. Let's find the coordinate locations of the photon sphere for massless particles and the ISCO for massive particles as functions of $m$, $a$, $F(r)$ and $G(r)$:

Consider the tangent vector to the worldline of a massive or massless particle, paramterized by some arbitrary affine parameter, $\lambda$:

\begin{equation}
    g_{ab}\frac{dx^{a}}{d\lambda}\frac{dx^{b}}{d\lambda}=-F(r)\left(\frac{dt}{d\lambda}\right)^{2}+G(r)\left(\frac{dr}{d\lambda}\right)^{2}+\left(r^{2}+a^{2}\right)\left\lbrace\left(\frac{d\theta}{d\lambda}\right)^{2}+\sin^{2}\theta \left(\frac{d\phi}{d\lambda}\right)^{2}\right\rbrace \ .
\end{equation}

\noindent As in the prior analysis, we may separate the two cases by defining a piecewise step function as follows:

\begin{equation}
    \epsilon = \left\{
    \begin{array}{rl}
    -1 & \qquad\mbox{Massive particle, \emph{i.e.} timelike worldline} \\
     0 & \qquad\mbox{Massless particle, \emph{i.e.} null geodesic} .
    \end{array}\right. 
\end{equation}

\noindent That is, $ds^{2}=\epsilon$, and due to the metric being spherically symmetric we may fix $\theta=\frac{\pi}{2}$ arbitrarily and view the reduced equatorial problem:
\begin{equation}
    g_{ab}\frac{dx^{a}}{d\lambda}\frac{dx^{b}}{d\lambda}=-F(r)\left(\frac{dt}{d\lambda}\right)^{2}+G(r)\left(\frac{dr}{d\lambda}\right)^{2}+\left(r^{2}+a^{2}\right)\left(\frac{d\phi}{d\lambda}\right)^{2}=\epsilon \ .
\end{equation}

\noindent Similarly to the Morris Thorne metric \ref{Morristhorne}, the Killing symmetries yield the following expressions for the conservation of energy $E$, and angular momentum $L$:

\begin{equation}
    F(r)\left(\frac{dt}{d\lambda}\right)=E \ ; \qquad\quad \left(r^{2}+a^{2}\right)\left(\frac{d\phi}{d\lambda}\right)=L \ .
\end{equation}

\noindent Hence:

\begin{equation}
    \frac{-E^2}{F(r)}+G(r)\left(\frac{dr}{d\lambda}\right)^2+\frac{L^{2}}{r^{2}+a^{2}}=\epsilon \ ,
\end{equation}
\\
\begin{equation}
    \Rightarrow\quad\left(\frac{dr}{d\lambda}\right)^{2}=\frac{1}{G(r)}\left\lbrace \epsilon-\frac{L^2}{r^2+a^2}+\frac{E^2}{F(r)}\right\rbrace \ .
\end{equation}  
\\

\noindent Noting that we may assume both the photon sphere and ISCO locations to correspond to geodesic orbits, \emph{i.e.} fixed $r$-coordinate, \emph {i.e.} $\frac{dr}{d\lambda}=0$, this gives ``effective potentials" for geodesic orbits as follows (``potentials" are proportional to $E^{2}$):

\begin{equation}
    V_{\epsilon}(r)=F(r)\left\lbrace -\epsilon+\frac{L^{2}}{r^{2}+a^{2}}\right\rbrace \ .
\end{equation}

%%

\begin{itemize}
    \item For a photon orbit we have the massless particle case $\epsilon=0$. Since we are in a spherically symmetric environment, solving for the locations of such orbits amounts to finding the coordinate location of the 'photon sphere'; \emph {i.e.} the value of the $r$-coordinate sufficiently close to our mass such that photons are forced to propogate in circular geodesic orbits. These circular orbits occur at $V_{0}^{'}(r)=0$ \red {(ref req?)}, as such:
    \begin{equation}
        V_{0}(r)=F(r)\left(\frac{L^{2}}{r^{2}+a^{2}}\right) \ ,
    \end{equation}
    leading to:
    \begin{equation}
        V_{0}^{'}(r)=\frac{L^2}{r^2+a^2}\left\lbrace \partial_{r}\left[F\left(r\right)\right]-\frac{2r}{r^2+a^2}\right\rbrace \ .
    \end{equation}
    When $V_{0}^{'}(r)=0$, this gives the location of these circular orbits as the $r$-values which solve the first order partial differential equation (recall that $F(r)$ is assumed to be given explicitly):
    
    \begin{equation}
        \partial_{r}\left[F\left(r\right)\right] = \frac{2r}{r^2+a^2} \ .
    \end{equation}
    
    \red {(discuss existence & uniqueness of sol's here, establish the necessary conditions on $F(r)$)}
    
    
    \noindent To verify stability, check the sign of $V_{0}^{''}(r)$:
    
    \red {(note $F(r)$ must be at least twice differentiable)}
    
    %%
    
    \item For massive particles the geodesic orbit corresponds to a timelike worldline and we have the case that $\epsilon=-1$. Therefore:
    \begin{equation}
        V_{-1}(r)=F(r)\left(1+\frac{L^{2}}{r^{2}+a^{2}}\right) \ ,
    \end{equation}
    and it is easily verified that this leads to:
    \begin{equation}
        V_{-1}^{'}(r)=\frac{L^2}{r^2+a^2}\left\lbrace \partial_{r}\left[F\left(r\right)\right]\left(1+\frac{r^2+a^2}{L^2}\right)-\frac{2r}{r^2+a^2}\right\rbrace \ .
    \end{equation}
    Equating this to zero amounts to solving the algebraic equation (given an explicit $F(r)$):
    \begin{equation}
        \partial_{r}\left[ F\left(r\right)\right] = \frac{2rL^2}{\left(r^2+a^2\right)\left(L^2+r^2+a^2\right)} \ .
    \end{equation}
\end{itemize}

%
\subsection{Regge-Wheeler}

\red {To be completed}

%
\subsection {Stress-energy-momentum tensor:}

\red{to be completed...}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> binding.tex <==
\chapter{Binding}\label{C:bin}

The Library states:
\begin{itemize}
\item Thesis must be fully bound and cased in cloth or buckram in optional colour. (I think they mean you can pick the colour!)
\item Author's surname and initials and (short) title lettered on spine. (The thesis's title, not the author's, presumably.)
\item Author's full name and full title lettered on front cover. (Again, the thesis's title, not the author's, presumably.)
\item Two copies of a PhD thesis and one copy of a Master's thesis must be deposited. A signed availability slip must accompany the thesis.
\item  The principal supervisor is responsible for the deposit.
\end{itemize}

==> library.tex <==
\chapter{Library requirements}\label{C:lib}

This Chapter describes some things done to be in accordance with the `Library Requirements for the Deposit of Theses' booklet, which can be obtained from the VUW library.

\section{Font size}
\textit{12 point font is recommended.} 

Set this yourself with the \verb+12pt+ option to the document class.

\section{Single or double sided}
\textit{Typing on one side preferred, text on both sides acceptable for longer works.} 

Use the \verb+oneside+ or \verb+twoside+ option to the document class. The \textsf{book} class default is \verb+twoside+.


\section{Line spacing}
\textit{Lines should be double spaced, or at least 1.5 spaces apart.} 

1.5 spacing for 12 point is set using:
\begin{itemize}
\item \verb+\renewcommand{\baselinestretch}{1.24}+  
\end{itemize}

To set anything else use, e.g  \verb+\renewcommand{\baselinestretch}{1.0}+ in the preamble. See p 53 of \cite{GMS94} for more information.


\section{Margins}
\textit{Uniform margins of at least 4cm on binding side, other three sides to have at least 1.5 cm}

\LaTeX\ styles often leave a lot of white space, and \textsf{book} is no exception. We only have to worry about the binding side.

For \verb+twoside+ we use these settings:
\setlength{\textheight}{19.8cm}
\setlength{\oddsidemargin}{1.46cm}
\setlength{\evensidemargin}{0.83cm}

For \verb+oneside+, if we use:
\begin{verbatim}
\setlength{\textheight}{19.8cm}
\setlength{\oddsidemargin}{1.46cm}
\end{verbatim}

Then \textsf{book} gives a margin of 4cm on the binding side, and about 3.2cm elsewhere.

If you want to change these then use the \textsf{layout} package.

\section{Paper size}
\textit{High quality A4 paper, all pages of equal size}

Set this yourself with the \verb+a4paper+ option to the document class.

==> thestyle.tex <==
\chapter{The front pages}\label{C:ex}

You can declare:
\begin{itemize}
\item an author using  \verb+\author{}+ -- your full name;
\item a title using \verb+\title{}+-- ALL IN CAPITALS IN THE EXAMPLE, but we use \verb#\Large# and \verb#\bf#, so normal case will do;
\item a subject using \verb+\subject{}+-- probably Computer Science, but you can pick anything you like;
\item an abstract using \verb+\abstract{}+-- this should be fewer then 500 words for a PhD. The handbook states ``A length of about 300 words is recommended.'' The \textsf{book} style does not have an \verb+abstract+ environment defined, so this is a bit of a hack.
\end{itemize}

You can also specify what degree you are submitting the thesis for by using:
\begin{itemize}
\item  \verb+\phd+, which produces ``\ldots in fulfilment of \ldots Doctor of Philosophy''
\item  \verb+\mscthesisonly+, which produces ``\ldots in fulfilment of \ldots Master of Science''
\item  \verb+\mscwithhonours+, which produces ``\ldots in partial fulfilment of \ldots Master of Science with Honours''
\item  \verb+\mscbothparts+, which produces ``\ldots in partial fulfilment of \ldots Master of Science''
\item  \verb+\otherdegree{DEGREE OR DIPLOMA NAME}+, which produces ``\ldots in fulfilment of \ldots DEGREE OR DIPLOMA NAME''
\end{itemize}

